Fast and Power Efficient Sensor Arbitration: Physical Layer Collision Recovery of Passive RFID Tags

This work concerns physical layer collision recovery for cheap sensors with allowed variations in frequency and delay of their communications. The work is presented as a generic, communication theoretic framework and demonstrated using UHF RFID tag technology. Previous work in this area has not provided recovery for more than two tags, which is shown to be possible in this work. Also presented is a novel mathematical model of the tag signal, incorporating the allowed variations in frequency and delay. The main motivation is seen in the observation that random variations in frequency and delay make the collided signals of different tags separable. The collision recovery is done by estimating the sensor specific variation in frequency and delay and using these estimates in a successive interference cancellation algorithm and a maximum likelihood sequence decoder, to iteratively reconstruct a sensor signal and remove it from the received signal. Numerical simulations show that the estimates and proposed algorithm are effective in recovering collisions. The proposed algorithm is then incorporated into a numerical simulation of the Qprotocol for UHF RFID tags and is shown to be effective in providing fast and power efficient sensor arbitration.

==> Makefile <==
DOC=collision_recov

TEXSOURCES=common.tex \
	collision_recov.tex
IMAGESOURCES=

all: $(DOC).pdf
ps: $(DOC).ps

$(DOC).dvi: $(TEXSOURCES) $(IMAGESOURCES) refs.bib
	latex $(DOC)
	latex $(DOC)
	latex $(DOC)
	bibtex $(DOC)
	latex $(DOC)
	latex $(DOC)

%.pdf: %.dvi
	dvipdf $< $@

clean:
	rm -rf *.idx *.aux *.log *.out *.toc *.bbl *.blg *.lof *.dvi $(DOC).ps $(DOC).pdf $(DOC).fff $(DOC).ttt

